Outfit Generation and Recommendation -- An Experimental Study

Over the past years, fashion-related challenges have gained a lot of attention in the research community. Outfit generation and recommendation, i.e., the composition of a set of items of different types (e.g., tops, bottom, shoes, accessories) that go well together, are among the most challenging ones. That is because items have to be both compatible amongst each other and also personalized to match the taste of the customer. Recently there has been a plethora of work targeted at tackling these problems by adopting various techniques and algorithms from the machine learning literature. However, to date, there is no extensive comparison of the performance of the different algorithms for outfit generation and recommendation. In this paper, we close this gap by providing a broad evaluation and comparison of various algorithms, including both personalized and non-personalized approaches, using online, real-world user data from one of Europe's largest fashion stores. We present the adaptations we made to some of those models to make them suitable for personalized outfit generation. Moreover, we provide insights for models that have not yet been evaluated on this task, specifically, GPT, BERT and Seq-to-Seq LSTM.

==> content/datasets.tex <==
\section{Datasets}
\label{sect:datasets}

In this section we present the datasets used to train and evaluate our models. They come from Zalando, a hub for digital fashion content in Europe. In the online shop, customers can purchase or seek for inspiration about garments and style via, for example, outfits.

The hand-crafted outfits we use to train our models are created in three different ways: (1) outfits from content creators (such as stylists) on the website (Shop the Look, STL), (2) influencer-created outfits (Get the Look, GTL)\footnote{\url{https://en.zalando.de/get-the-look-women}}, where influencers assemble their own outfits, and (3) via Zalando's personalized styling service Zalon\footnote{\url{https://zalon.de}} where stylists create outfits customized for each customer individually.

\begin{itemize}

\item \textbf{Zalando outfit dataset (GTL and STL)}: This dataset consists of around 250k hand-created outfits that have been published on Zalando, containing a total of 1M distinct items. This includes STL styled by Zalando creators, provided as an inspirational supplement to the item on the product detail page, and the influencer-created outfits available on GTL. Each of these outfits is composed of a single item per body part that can be worn together, occasionally accompanied by a fashion accessory.

\item \textbf{Zalon outfit dataset}: A dataset of around 380k recent outfits, each of which has been handcrafted for a specific customer by a professional stylist. A Zalon stylist assembles an outfit based on \emph{questionnaire} answers that a customer provides, where they express their style preferences, provide body features to the stylist, and specify price expectations. Based on this information, the stylist creates a personalized box consisting of two outfits, where each consists of up to seven articles, for example shoes, pants, t-shirt, sweater, and jacket. There can be multiple articles of one type, for example multiple pants or tops, but all of them are compatible amongst each other. Zalon's dataset contains about 30k distinct articles from the Zalando fashion store. To restrict ourselves to this limited set of distinct articles, we removed the long tail of articles which appear less than eight items.

\end{itemize}

In Table~\ref{table:outfitdataset} we show a summary of the two outfit datasets we just described. With the previous datasets, we can solve the compatibility problem. However, in order to be able to cater for the specific taste of our customers, we also make use of customer context. The following two datasets contain user specific data in the form of clicks and questionnaires:

\begin{table}
    \caption{Comparison of the key properties of Zalando's GTL \& STL and Zalon's outfit dataset.}
    \label{table:outfitdataset}
    \begin{tabular}{l l r r r}
        \toprule
        Dataset & Personalization & \#Outfits & \#Articles & Avg. outfit length \\
        \midrule
        Zalando GTL \& STL & Click history & 251,891 & 64,748 & 4.50 articles \\
        Zalon & Questionnaire & 380,808 & 30,619 & 4.96 articles \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{itemize}

\item \textbf{Zalando click dataset}: This dataset consists of user click actions (clicks on articles, additions to the wishlist, etc.) on a single item and user actions on whole outfits that are available on Zalando. In total there are close to 1M outfits per year created on the Zalando web page available to approximately 32M active customers. We aggregate the past actions per user over a period of one month and create training samples consisting of outfit interactions together with the preceding item actions such as click and add-to-wishlist. The outfit actions are taken into consideration only if there are at least five item actions preceding it and contain at least four items, excluding accessories. We exclude fashion items that are rare and occur less than three times in the action data. This way, we obtain around 6M valid training samples that contain around 200k distinct outfits and 100k distinct items.

\item \textbf{Zalon questionnaire dataset}: In Zalon, each customer that requests a personalized outfit needs to fill a detailed questionnaire, which gives information about style preferences, provides body features to the stylist, and specifies price expectations. The total number of features we collect is over 30, with some examples of questionnaire fields being the shoe size, no-go dress types, favorite brands, favorite colors, hair color, body height and weight, and the occasion for which an outfit is needed. The total amount of questionnaires for training our models is around~250k.

\end{itemize}

Our datasets are proprietary and cannot be released for customer privacy reasons. The Zalon dataset is distinct from other datasets in the domain because of its rich questionnaire features which contain significantly more information about a customer than their click or purchase history. It is therefore especially promising to use in combination with personalized models.

